Clustering of functional data prone to complex heteroscedastic measurement error

Several factors make clustering of functional data challenging, including the infinite-dimensional space to which observations belong and the lack of a defined probability density function for the functional random variable. To overcome these barriers, researchers either assume that observations belong to a finite-dimensional space spanned by basis functions or apply nonparametric smoothing methods to the functions prior to clustering. Although extensive literature describes clustering methods for functional data, few studies have explored the clustering of measurement error--prone function-valued data. In this work, we consider clustering methods for functional data prone to complex, heteroscedastic measurement errors. Two stage-based methods using mixed-effects models are first applied to adjust for measurement error bias, followed by cluster analysis of the measurement error--adjusted curves. Through simulations, we investigate how varying sample size, the magnitude of measurement error, and the presence of complex heteroscedastic measurement errors influence the cluster analysis of functional data. Our results indicate that failing to account for measurement errors and the correlation structures associated with frequently collected functional data reduces the accuracy of identifying the true latent groups or clusters. The method consistently produces better results regardless of the initial clustering values used. Moreover, it is flexible and can be applied to various clustering approaches, based on the specific distribution of the data. The developed methods are applied to two data sets: a school-based study of energy expenditure among elementary school-aged children in Texas and data from the National Health and Nutrition Examination Survey on participants' physical activity monitored by wearable devices at frequent intervals.

==> draft.tex <==
Ma et al. proposed smoothing spline clustering model to capture natural properties of gene expression over time. They employed a mixed effect model to account for measurement error, subject-specific effect and clustered-specific effect. Next, they maximized the summation of the penalized log-likelihood, considering the correlation between time points. The authors came up with a rejection-controlled process based on basic Expectation-Maximization method to update the posterior probability of each gene $i$ belong to cluster $k$ [\cite{ma2006data}]. However, the mean curve of each cluster was derived from all time points, which could smooth out important variations in individual trajectories. Physical activity data often have high variability, including non-linear patterns, sharp changes, or irregular time intervals[\cite{farrahi2024machine}].
